Self-adaptive absorbing boundary conditions for quasilinear acoustic wave propagation

We propose a self-adaptive absorbing technique for quasilinear ultrasound waves in two- and three-dimensional computational domains. As a model for the nonlinear ultrasound propagation in thermoviscous fluids, we employ Westervelt's wave equation solved for the acoustic velocity potential. The angle of incidence of the wave is computed based on the information provided by the wave-field gradient which is readily available in the finite element framework. The absorbing boundary conditions are then updated with the angle values in real time. Numerical experiments illustrate the accuracy and efficiency of the proposed method.

==> images/Horn3D/Cost_V.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.60000,0.00000}%
%
\begin{tikzpicture}[scale = 0.52, font=\huge]

\begin{axis}[%
width=4.602in,
height=3.82in,
at={(0.772in,0.516in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\huge\color{white!15!black}},
xlabel={relative simulation time $t/T$}, xtick={0, 0.2, 0.4, 0.6, 0.8, 1},
y tick label style={
        /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=2,
        /tikz/.cd
            },
ymin=0.02,
ymax=0.18,
ylabel style={font=\huge\color{white!15!black}},
ylabel={relative $L^{2}(\Omega)$ error},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
0.00476190476190474	0.176204169574423\\
0.00929705215419496	0.0992555609928991\\
0.0138321995464853	0.0733091827583424\\
0.0183673469387755	0.0510292060302791\\
0.0229024943310657	0.0412429255267689\\
0.0274376417233561	0.0500973315975423\\
0.0319727891156463	0.0749340386961795\\
0.0365079365079365	0.0910741868531351\\
0.0410430839002267	0.0727187251002612\\
0.045578231292517	0.0486017126532667\\
0.0501133786848073	0.0336471048126967\\
0.0546485260770975	0.0271415842970067\\
0.0591836734693878	0.0278333766800226\\
0.063718820861678	0.034395185704487\\
0.0682539682539682	0.0435973965551958\\
0.0727891156462586	0.0520609791732861\\
0.0773242630385488	0.0530564268797749\\
0.081859410430839	0.044451555544514\\
0.0863945578231292	0.0333658488399958\\
0.0909297052154195	0.0262199890980311\\
0.0954648526077098	0.0249503908095042\\
0.1	0.0280464795776553\\
0.10453514739229	0.0330586258095431\\
0.109070294784581	0.0383707970057634\\
0.113605442176871	0.042092551582119\\
0.118140589569161	0.0417635037730985\\
0.122675736961451	0.0367656502174328\\
0.127210884353742	0.0303156961764052\\
0.131746031746032	0.0262790436825339\\
0.136281179138322	0.0259241796670446\\
0.140816326530612	0.0281983786662419\\
0.149886621315193	0.0350884302812638\\
0.154421768707483	0.0374679268310342\\
0.158956916099773	0.0374852763808403\\
0.163492063492063	0.0344734134888129\\
0.168027210884354	0.0299337303337831\\
0.172562358276644	0.0267053141658236\\
0.177097505668934	0.0288114813273775\\
0.181632653061225	0.0328727395826118\\
0.186167800453515	0.0367156917473774\\
0.190702947845805	0.037935636034934\\
0.195238095238095	0.0377531410899178\\
0.199773242630386	0.0368705358095085\\
0.204308390022676	0.0350786263880027\\
0.208843537414966	0.0318056915569596\\
0.213378684807256	0.0304114584551741\\
0.217913832199547	0.0310790461336183\\
0.222448979591837	0.033133622811465\\
0.226984126984127	0.0337940468140131\\
0.231519274376417	0.0337522186256779\\
0.236054421768708	0.0331129645100164\\
0.240589569160998	0.0319183030644269\\
0.245124716553288	0.0292982544641736\\
0.249659863945578	0.0271220285914384\\
0.254195011337868	0.0266179498029766\\
0.258730158730159	0.027529671850743\\
0.263265306122449	0.0289693792932877\\
0.267800453514739	0.0301739564607232\\
0.272335600907029	0.0310425265577726\\
0.27687074829932	0.0306279026291175\\
0.28140589569161	0.0287985548804175\\
0.2859410430839	0.0263203687269919\\
0.290476190476191	0.0240797724807195\\
0.295011337868481	0.0236863538330494\\
0.299546485260771	0.0247884595195875\\
0.304081632653061	0.0264897968279141\\
0.308616780045352	0.0283109093075473\\
0.313151927437642	0.029124384610213\\
0.317687074829932	0.0286649449244972\\
0.322222222222222	0.0270909409839331\\
0.326757369614513	0.0247668447147045\\
0.331292517006803	0.0229693129722075\\
0.335827664399093	0.0230356754493224\\
0.340362811791383	0.0242025929383607\\
0.344897959183673	0.0261254379979431\\
0.349433106575964	0.0279634994512422\\
0.353968253968254	0.0288570470248187\\
0.358503401360544	0.0287494418111738\\
0.363038548752834	0.0278027199439728\\
0.367573696145125	0.0263105071633954\\
0.372108843537415	0.0251010695527722\\
0.376643990929705	0.0247688115783468\\
0.381179138321995	0.0255511829074907\\
0.385714285714286	0.0267598935596434\\
0.390249433106576	0.028385030835313\\
0.394784580498866	0.0291869132484742\\
0.399319727891156	0.0294866737276519\\
0.403854875283447	0.0289206238194921\\
0.408390022675737	0.0280422944297969\\
0.412925170068027	0.0276321108943826\\
0.417460317460318	0.0277447598504474\\
0.421995464852608	0.0287855917875632\\
0.426530612244898	0.0302732002327559\\
0.431065759637188	0.0319378548867748\\
0.435600907029479	0.0331938445272073\\
0.440136054421769	0.0338665864108083\\
0.444671201814059	0.0340495093518585\\
0.449206349206349	0.0340389466041435\\
0.45827664399093	0.0348767694660196\\
0.46281179138322	0.0357966065322461\\
0.46734693877551	0.0368342845413623\\
0.4718820861678	0.0377934251567209\\
0.476417233560091	0.0384524302900183\\
0.480952380952381	0.0388524867669594\\
0.490022675736961	0.0394346684391025\\
0.494557823129252	0.0399804486231757\\
0.499092970521542	0.0408324032753405\\
0.508163265306122	0.0429990195319203\\
0.512698412698413	0.0438532762664938\\
0.517233560090703	0.044237184503868\\
0.526303854875283	0.0445670532545654\\
0.530839002267574	0.0448849089176986\\
0.535374149659864	0.0456707199097593\\
0.539909297052154	0.0468735906222193\\
0.544444444444444	0.0482911604884867\\
0.548979591836735	0.0492073020586864\\
0.553514739229025	0.0493483979776486\\
0.558049886621315	0.048953819132182\\
0.562585034013605	0.0484788751362845\\
0.567120181405896	0.0486587917537149\\
0.571655328798186	0.0498854894798694\\
0.576190476190476	0.0513136010169049\\
0.580725623582766	0.0526554719171484\\
0.585260770975057	0.0535271992837246\\
0.589795918367347	0.0534549371713049\\
0.594331065759637	0.052519129366528\\
0.598866213151927	0.05199565623402\\
0.603401360544218	0.0520182661554897\\
0.607936507936508	0.0528357253430994\\
0.617006802721088	0.0563876995090576\\
0.621541950113379	0.0574122011475386\\
0.626077097505669	0.0577221708489521\\
0.630612244897959	0.0568269764758578\\
0.635147392290249	0.0548793154339368\\
0.63968253968254	0.0535975075158566\\
0.64421768707483	0.0537812472703673\\
0.64875283446712	0.0553539611995936\\
0.657823129251701	0.0612567779054977\\
0.662358276643991	0.0626477886920878\\
0.666893424036281	0.0621848651616778\\
0.671428571428571	0.0598210581594572\\
0.675963718820862	0.0559646310288533\\
0.680498866213152	0.0529432495966411\\
0.685034013605442	0.0531191385342343\\
0.689569160997732	0.056223340105124\\
0.694104308390023	0.0609207767879519\\
0.698639455782313	0.0652070974931191\\
0.703174603174603	0.0672347433641348\\
0.707709750566893	0.0663149006252465\\
0.712244897959184	0.0629708372618997\\
0.716780045351474	0.0578904195844352\\
0.721315192743764	0.0531963011375661\\
0.725850340136054	0.0520722816323167\\
0.730385487528345	0.0551700543387814\\
0.734920634920635	0.0606197564080561\\
0.739455782312925	0.0661604992702448\\
0.743990929705215	0.0695434623067479\\
0.748526077097506	0.0695057580331681\\
0.753061224489796	0.0662614112657245\\
0.757596371882086	0.060601401486556\\
0.762131519274376	0.0543104000498573\\
0.766666666666667	0.050932004215\\
0.771201814058957	0.0530541480851721\\
0.775736961451247	0.0588317076314593\\
0.780272108843537	0.06547439073913\\
0.784807256235828	0.0704413985244011\\
0.789342403628118	0.0718960513599605\\
0.793877551020408	0.0695485114365898\\
0.798412698412698	0.0642182866072979\\
0.802947845804989	0.0571759641493247\\
0.807482993197279	0.0514279452089521\\
0.812018140589569	0.0510372268751207\\
0.816553287981859	0.0561034259944726\\
0.82108843537415	0.0632637884998332\\
0.82562358276644	0.0695309040704223\\
0.83015873015873	0.072734871658354\\
0.83469387755102	0.0717734703057653\\
0.839229024943311	0.0672484946051128\\
0.848299319727891	0.0536974967149153\\
0.852834467120181	0.0507938627823631\\
0.857369614512472	0.0539633907666689\\
0.861904761904762	0.0605174885822419\\
0.866439909297052	0.0671970015502181\\
0.870975056689342	0.072020306723695\\
0.875510204081633	0.0733033519139489\\
0.880045351473923	0.0708625965246338\\
0.884580498866213	0.065626573459475\\
0.889115646258503	0.0587739618576771\\
0.893650793650794	0.0532648372306244\\
0.898185941043084	0.0528997919020741\\
0.902721088435374	0.0576478324527904\\
0.907256235827664	0.0643062640614334\\
0.911791383219955	0.0704937077130861\\
0.916326530612245	0.0741162676850584\\
0.920861678004535	0.073804059685135\\
0.925396825396825	0.070084138731203\\
0.929931972789116	0.0639688724201424\\
0.934467120181406	0.0571222649218429\\
0.939002267573696	0.0533353956405562\\
0.943537414965986	0.0554876630793082\\
0.948072562358277	0.0615182559439641\\
0.952607709750567	0.0682386151517325\\
0.957142857142857	0.0737634691215587\\
0.961678004535147	0.0762009576208655\\
0.966213151927438	0.0746944891173196\\
0.970748299319728	0.0698912326643496\\
0.975283446712018	0.0630615324387558\\
0.979818594104308	0.0567672153666631\\
0.984353741496599	0.0551891935447476\\
0.988888888888889	0.0592206058015085\\
0.993424036281179	0.065990911128326\\
0.997959183673469	0.0729731955319129\\
};
\addlegendentry{ABC$_W^{1/2}$ adaptive}

\addplot [color=mycolor1, dashed]
  table[row sep=crcr]{%
0.00476190476190474	0.176204169574423\\
0.00929705215419496	0.0992555609928991\\
0.0138321995464853	0.0733091827583424\\
0.0183673469387755	0.0510292060302791\\
0.0229024943310657	0.0412429255267689\\
0.0274376417233561	0.0500973315975423\\
0.0319727891156463	0.0749340386961795\\
0.0365079365079365	0.0910741868531351\\
0.0410430839002267	0.0727187251002612\\
0.045578231292517	0.0486017126532667\\
0.0501133786848073	0.0336471048126967\\
0.0546485260770975	0.0271415842970067\\
0.0591836734693878	0.0278333766800226\\
0.063718820861678	0.034395185704487\\
0.0682539682539682	0.0435973965551958\\
0.0727891156462586	0.0520609791732861\\
0.0773242630385488	0.0530564268797749\\
0.081859410430839	0.044451555544514\\
0.0863945578231292	0.0333658488399958\\
0.0909297052154195	0.0262199890980311\\
0.0954648526077098	0.0249503908095042\\
0.1	0.0280464795776553\\
0.10453514739229	0.0330586258095431\\
0.109070294784581	0.0383707970057634\\
0.113605442176871	0.042092551582119\\
0.118140589569161	0.0417635037730985\\
0.122675736961451	0.0367656502174328\\
0.127210884353742	0.0303156961764052\\
0.131746031746032	0.0262790436825339\\
0.136281179138322	0.0259241796670446\\
0.140816326530612	0.0281983786662419\\
0.149886621315193	0.0350884302812638\\
0.154421768707483	0.0374679268310342\\
0.158956916099773	0.0374852763808403\\
0.163492063492063	0.0344734134888129\\
0.168027210884354	0.0299337303337831\\
0.172562358276644	0.0267053141658236\\
0.177097505668934	0.0288114813273775\\
0.181632653061225	0.0328727395826118\\
0.186167800453515	0.0367156917473774\\
0.190702947845805	0.037935636034934\\
0.195238095238095	0.0377531410899178\\
0.199773242630386	0.0368705358095085\\
0.204308390022676	0.0350786263880027\\
0.208843537414966	0.0318056915569596\\
0.213378684807256	0.0304114584551741\\
0.217913832199547	0.0310790461336183\\
0.222448979591837	0.033133622811465\\
0.226984126984127	0.0337940468140131\\
0.231519274376417	0.0337522186256779\\
0.236054421768708	0.0331129645100164\\
0.240589569160998	0.0319183030644269\\
0.245124716553288	0.0292982544641736\\
0.249659863945578	0.0271220285914384\\
0.254195011337868	0.0266179498029766\\
0.258730158730159	0.027529671850743\\
0.263265306122449	0.0289693792932877\\
0.267800453514739	0.0301739564607232\\
0.272335600907029	0.0310425265577726\\
0.27687074829932	0.0306279026291175\\
0.28140589569161	0.0287985548804175\\
0.2859410430839	0.0263203687269919\\
0.290476190476191	0.0240797724807195\\
0.295011337868481	0.0236863538330494\\
0.299546485260771	0.0247884595195875\\
0.304081632653061	0.0264897968279141\\
0.308616780045352	0.0283109093075473\\
0.313151927437642	0.029124384610213\\
0.317687074829932	0.0286649449244972\\
0.322222222222222	0.0270909409839331\\
0.326757369614513	0.0247668447147045\\
0.331292517006803	0.0229693129722075\\
0.335827664399093	0.0230356754493224\\
0.340362811791383	0.0242025929383607\\
0.344897959183673	0.0261254379979431\\
0.349433106575964	0.0279634994512422\\
0.353968253968254	0.0288570470248187\\
0.358503401360544	0.0287494418111738\\
0.363038548752834	0.0278027199439728\\
0.367573696145125	0.0263105071633954\\
0.372108843537415	0.0251010695527722\\
0.376643990929705	0.0247679200252605\\
0.381179138321995	0.0255326340713684\\
0.385714285714286	0.0267022114815316\\
0.390249433106576	0.028260024956405\\
0.394784580498866	0.028990291142739\\
0.399319727891156	0.02918384997935\\
0.403854875283447	0.0285358520367781\\
0.408390022675737	0.0274765935498213\\
0.412925170068027	0.026894379114236\\
0.417460317460318	0.0267774719858136\\
0.421995464852608	0.0275794421595815\\
0.426530612244898	0.028818235912328\\
0.431065759637188	0.0302910638712887\\
0.435600907029479	0.0313912532050789\\
0.440136054421769	0.031998739841936\\
0.444671201814059	0.0320866894033525\\
0.449206349206349	0.0320015948972985\\
0.453741496598639	0.0323311106492066\\
0.45827664399093	0.0326022439279455\\
0.46281179138322	0.0334287436707464\\
0.46734693877551	0.0345013353707921\\
0.4718820861678	0.0357400664854396\\
0.476417233560091	0.0366892969439315\\
0.480952380952381	0.037475572387486\\
0.485487528344671	0.0381310385098108\\
0.490022675736961	0.0385777770626755\\
0.494557823129252	0.039166682886915\\
0.499092970521542	0.0399972319819566\\
0.503628117913832	0.0410610821771926\\
0.508163265306122	0.0423365729467974\\
0.512698412698413	0.0435166448932576\\
0.517233560090703	0.0443034986759753\\
0.530839002267574	0.0460911135319614\\
0.535374149659864	0.0469273508441129\\
0.539909297052154	0.0481440815319241\\
0.548979591836735	0.0510826211913094\\
0.553514739229025	0.0520517769578004\\
0.558049886621315	0.0523437002242348\\
0.567120181405896	0.051803683166201\\
0.571655328798186	0.0520925220530045\\
0.576190476190476	0.0532569767570762\\
0.580725623582766	0.0554663518729684\\
0.585260770975057	0.058046708964917\\
0.589795918367347	0.0600470577685953\\
0.594331065759637	0.0604029074773631\\
0.598866213151927	0.0591639046348985\\
0.603401360544218	0.0568564254715958\\
0.607936507936508	0.0547773445484839\\
0.612471655328798	0.0546071288964245\\
0.617006802721088	0.0570811773824503\\
0.621541950113379	0.0616263584784276\\
0.626077097505669	0.0666135599591173\\
0.630612244897959	0.0698472675544001\\
0.635147392290249	0.0697774869628289\\
0.63968253968254	0.0662066102941518\\
0.64421768707483	0.0604023686670078\\
0.64875283446712	0.0549345091037681\\
0.65328798185941	0.0532845265229578\\
0.657823129251701	0.0570751680117597\\
0.662358276643991	0.0647615264416703\\
0.666893424036281	0.0728635469759428\\
0.671428571428571	0.0782789338903517\\
0.675963718820862	0.0790666337996947\\
0.680498866213152	0.074748940512814\\
0.685034013605442	0.066414236369448\\
0.689569160997732	0.0570328754684134\\
0.694104308390023	0.0515426267437019\\
0.698639455782313	0.0540442274112705\\
0.703174603174603	0.0635139392074847\\
0.707709750566893	0.0748789089748185\\
0.712244897959184	0.0836980942311871\\
0.716780045351474	0.0869570655157321\\
0.721315192743764	0.0834822781801066\\
0.725850340136054	0.0739376930122586\\
0.730385487528345	0.061221845878807\\
0.734920634920635	0.0510171015472457\\
0.739455782312925	0.0503390834294396\\
0.743990929705215	0.0598161803231264\\
0.748526077097506	0.0731889519496408\\
0.753061224489796	0.0846357441075928\\
0.757596371882086	0.0906375894569503\\
0.762131519274376	0.0895262734402876\\
0.766666666666667	0.0814233207085824\\
0.771201814058957	0.0685087623138136\\
0.775736961451247	0.0553007088216982\\
0.780272108843537	0.0493304842100535\\
0.784807256235828	0.0553860967956882\\
0.793877551020408	0.082211843824224\\
0.798412698412698	0.0912628549771869\\
0.802947845804989	0.0933928681507546\\
0.807482993197279	0.0879346038833906\\
0.812018140589569	0.0761265578372516\\
0.816553287981859	0.0615921033363889\\
0.82108843537415	0.0510211900325942\\
0.82562358276644	0.0518217528476049\\
0.83015873015873	0.0631624667336397\\
0.83469387755102	0.077456613284703\\
0.839229024943311	0.0889276771406917\\
0.843764172335601	0.0943884673010564\\
0.848299319727891	0.0924351235004378\\
0.852834467120181	0.0834140283447125\\
0.861904761904762	0.0560037374803346\\
0.866439909297052	0.0502849563756199\\
0.870975056689342	0.0572979203565226\\
0.875510204081633	0.0715151061088896\\
0.880045351473923	0.0854183666209128\\
0.884580498866213	0.094435476332403\\
0.889115646258503	0.096199839489447\\
0.893650793650794	0.0901784579280095\\
0.898185941043084	0.0776113110732046\\
0.902721088435374	0.0623289937455321\\
0.907256235827664	0.0515273755302624\\
0.911791383219955	0.0532052642291498\\
0.916326530612245	0.0657395240567994\\
0.920861678004535	0.0807807963846098\\
0.925396825396825	0.0925468068805241\\
0.929931972789116	0.0977547811994689\\
0.934467120181406	0.0950844564303395\\
0.939002267573696	0.0849752562667789\\
0.943537414965986	0.0701034270261447\\
0.948072562358277	0.0561336804148028\\
0.952607709750567	0.0516001523899896\\
0.957142857142857	0.0604594808164322\\
0.961678004535147	0.0757869429506348\\
0.966213151927438	0.089891107233626\\
0.970748299319728	0.0984563158114286\\
0.975283446712018	0.0994323801431385\\
0.979818594104308	0.0923673655220094\\
0.984353741496599	0.0788571404627029\\
0.988888888888889	0.0632258137491055\\
0.993424036281179	0.053477940758851\\
0.997959183673469	0.0573674958025675\\
};
\addlegendentry{ABC$_W^{1/2}$}

\end{axis}
\end{tikzpicture}%

==> images/Horn3D/Cost_V_abs.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.60000,0.00000}%
%
\begin{tikzpicture}[scale = 0.52, font=\huge]

\begin{axis}[%
width=4.602in,
height=3.82in,
at={(0.772in,0.516in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\huge\color{white!15!black}},
xlabel={relative simulation time $t/T$}, xtick={0, 0.2, 0.4, 0.6, 0.8, 1},
y tick label style={
        /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=2,
        /tikz/.cd
            },
ymin=0,
ymax=0.45,
ylabel style={font=\huge\color{white!15!black}},
ylabel={absolute $L^{2}(\Omega)$ error},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
0.000226757369614528	0\\
0.0274376417233561	0.00105946340664176\\
0.0410430839002267	0.00261727556642299\\
0.0546485260770975	0.00282510768591271\\
0.0591836734693878	0.00342795032571575\\
0.063718820861678	0.00462557141214504\\
0.0727891156462586	0.00727366183501266\\
0.0773242630385488	0.00804729068665844\\
0.081859410430839	0.00821199666280259\\
0.0863945578231292	0.00790807147615624\\
0.0909297052154195	0.00780313069382887\\
0.0954648526077098	0.00885002433216642\\
0.1	0.0111834017579875\\
0.10453514739229	0.0140321973312689\\
0.109070294784581	0.0166299119386963\\
0.113605442176871	0.0183751051772724\\
0.118140589569161	0.0189539188548269\\
0.122675736961451	0.0185365200047953\\
0.127210884353742	0.0178856728879726\\
0.131746031746032	0.0182875558606923\\
0.136281179138322	0.0207525332872107\\
0.140816326530612	0.0249641225232572\\
0.145351473922902	0.0297013768897935\\
0.149886621315193	0.0337782207439414\\
0.154421768707483	0.0363092686417221\\
0.158956916099773	0.036951577703303\\
0.163492063492063	0.0359625337429585\\
0.168027210884354	0.0345866074703388\\
0.172562358276644	0.0349585812623219\\
0.177097505668934	0.0417023425437344\\
0.181632653061225	0.0511230847653164\\
0.186167800453515	0.0594305507756187\\
0.190702947845805	0.0623781475502696\\
0.195238095238095	0.0623902527038722\\
0.199773242630386	0.0615254894345335\\
0.204308390022676	0.0600491371989617\\
0.208843537414966	0.0569335578685286\\
0.213378684807256	0.0575817048501766\\
0.217913832199547	0.0621809306185614\\
0.222448979591837	0.0693231161364491\\
0.226984126984127	0.0728851738713047\\
0.231519274376417	0.0739764213884374\\
0.236054421768708	0.0730384208285301\\
0.240589569160998	0.0706594255106227\\
0.245124716553288	0.0654823244141816\\
0.249659863945578	0.0618648960646255\\
0.254195011337868	0.062635050149912\\
0.258730158730159	0.0671695900325606\\
0.263265306122449	0.0731180684615076\\
0.267800453514739	0.0781603846239197\\
0.272335600907029	0.0816945359553225\\
0.27687074829932	0.0811714143862393\\
0.28140589569161	0.0764950084494338\\
0.2859410430839	0.0701505858342022\\
0.290476190476191	0.0648425606396117\\
0.295011337868481	0.0649941211816527\\
0.299546485260771	0.0697722119666847\\
0.304081632653061	0.0765700008815974\\
0.308616780045352	0.0837059340787943\\
0.313151927437642	0.0874435224755171\\
0.317687074829932	0.086739535014926\\
0.322222222222222	0.0821723863246493\\
0.326757369614513	0.0752187922851598\\
0.331292517006803	0.0700976346722377\\
0.335827664399093	0.0711168005015608\\
0.340362811791383	0.0760743475284771\\
0.349433106575964	0.0916154838289017\\
0.353968253968254	0.0960115251749589\\
0.358503401360544	0.0964985605882963\\
0.363038548752834	0.0935989153619589\\
0.367573696145125	0.0885996862822129\\
0.372108843537415	0.0846574654364893\\
0.376643990929705	0.0840719297551169\\
0.381179138321995	0.0878145529386996\\
0.385714285714286	0.0935341773977798\\
0.390249433106576	0.1009979734815\\
0.394784580498866	0.105418934987751\\
0.399319727891156	0.107513107468945\\
0.403854875283447	0.105851666635349\\
0.408390022675737	0.102636182323638\\
0.412925170068027	0.101069819778461\\
0.417460317460318	0.101729625321995\\
0.421995464852608	0.106367584408419\\
0.426530612244898	0.113300624869032\\
0.431065759637188	0.121350975476631\\
0.435600907029479	0.127893406805641\\
0.440136054421769	0.131768153493184\\
0.444671201814059	0.13304878688018\\
0.449206349206349	0.132970734746081\\
0.453741496598639	0.134212211482304\\
0.45827664399093	0.135773208605719\\
0.46281179138322	0.13979176778833\\
0.46734693877551	0.145016812088777\\
0.4718820861678	0.150542059759152\\
0.476417233560091	0.155050238747933\\
0.480952380952381	0.158131740144671\\
0.485487528344671	0.160083730931429\\
0.490022675736961	0.161071889682118\\
0.494557823129252	0.162627629343276\\
0.499092970521542	0.165343397491555\\
0.503628117913832	0.169432722163604\\
0.512698412698413	0.179139186424187\\
0.517233560090703	0.182371989820673\\
0.521768707482993	0.184379808109336\\
0.526303854875283	0.185923620058736\\
0.530839002267574	0.187105836947943\\
0.535374149659864	0.189487295123921\\
0.539909297052154	0.193258336359823\\
0.544444444444444	0.198128183245969\\
0.548979591836735	0.201687782474291\\
0.553514739229025	0.203016289889412\\
0.558049886621315	0.202801847574645\\
0.562585034013605	0.202357677379379\\
0.567120181405896	0.204133533504431\\
0.576190476190476	0.21459012240706\\
0.580725623582766	0.218722469369719\\
0.585260770975057	0.220842528980863\\
0.589795918367347	0.219705569244842\\
0.594331065759637	0.216057513923489\\
0.598866213151927	0.214988895746586\\
0.603401360544218	0.216597670119097\\
0.607936507936508	0.221285477648803\\
0.612471655328798	0.229339777723396\\
0.617006802721088	0.236151877910148\\
0.621541950113379	0.239056820723474\\
0.626077097505669	0.238650858665816\\
0.630612244897959	0.233725025965786\\
0.635147392290249	0.225475454015281\\
0.63968253968254	0.221024143268941\\
0.64421768707483	0.223291536885614\\
0.64875283446712	0.23143895029985\\
0.65328798185941	0.244881045791921\\
0.657823129251701	0.25714361945795\\
0.662358276643991	0.261775190574642\\
0.666893424036281	0.258011010664168\\
0.671428571428571	0.246577752587758\\
0.675963718820862	0.229923031567425\\
0.680498866213152	0.217785451726363\\
0.685034013605442	0.219648373621607\\
0.689569160997732	0.234033952578288\\
0.694104308390023	0.254907508306078\\
0.698639455782313	0.273299547043166\\
0.703174603174603	0.281066696109068\\
0.707709750566893	0.275595521835652\\
0.712244897959184	0.259925673101805\\
0.716780045351474	0.237798372270886\\
0.721315192743764	0.218347855566754\\
0.725850340136054	0.214520076505212\\
0.730385487528345	0.22879760139105\\
0.739455782312925	0.277285392648285\\
0.743990929705215	0.291331442173862\\
0.748526077097506	0.289874162695604\\
0.753061224489796	0.27450654405551\\
0.757596371882086	0.249510286884125\\
0.762131519274376	0.222935927511477\\
0.766666666666667	0.209328465677643\\
0.771201814058957	0.219114449538506\\
0.775736961451247	0.244503803899667\\
0.780272108843537	0.273462027005036\\
0.784807256235828	0.294695683970201\\
0.789342403628118	0.300082616906917\\
0.793877551020408	0.288746610782427\\
0.798412698412698	0.264945675907918\\
0.802947845804989	0.234807160868317\\
0.807482993197279	0.210999921907161\\
0.812018140589569	0.210044796939913\\
0.816553287981859	0.23225847821483\\
0.82108843537415	0.2635248320173\\
0.82562358276644	0.290807566791256\\
0.83015873015873	0.304282338830968\\
0.83469387755102	0.299183891360829\\
0.839229024943311	0.278628950581577\\
0.848299319727891	0.220406327739405\\
0.852834467120181	0.208579992397854\\
0.857369614512472	0.222479297081239\\
0.866439909297052	0.280017484676008\\
0.870975056689342	0.300858726617927\\
0.875510204081633	0.305889084992829\\
0.880045351473923	0.294430341338846\\
0.884580498866213	0.271011219090567\\
0.889115646258503	0.241402635679613\\
0.893650793650794	0.218269627687669\\
0.898185941043084	0.217197836917709\\
0.902721088435374	0.23798055446564\\
0.907256235827664	0.267261872304003\\
0.911791383219955	0.294525973719039\\
0.916326530612245	0.310117934360643\\
0.920861678004535	0.307892674732948\\
0.925396825396825	0.290538095898502\\
0.929931972789116	0.263361281144977\\
0.934467120181406	0.234091998192073\\
0.939002267573696	0.218480984782153\\
0.943537414965986	0.22816769166869\\
0.948072562358277	0.254565762284416\\
0.952607709750567	0.284108516631075\\
0.957142857142857	0.308165640613329\\
0.961678004535147	0.31811307004416\\
0.966213151927438	0.310321928933199\\
0.970748299319728	0.288319879867803\\
0.975283446712018	0.258487548570346\\
0.979818594104308	0.232026834033057\\
0.984353741496599	0.226031293528644\\
0.988888888888889	0.244041329247414\\
0.997959183673469	0.304886576826023\\
};
\addlegendentry{ABC$_W^{1/2}$ adaptive}

\addplot [color=mycolor1, dashed]
  table[row sep=crcr]{%
0.000226757369614528	0\\
0.0274376417233561	0.00105946340664176\\
0.0410430839002267	0.00261727556642299\\
0.0546485260770975	0.00282510768591271\\
0.0591836734693878	0.00342795032571575\\
0.063718820861678	0.00462557141214504\\
0.0727891156462586	0.00727366183501266\\
0.0773242630385488	0.00804729068665844\\
0.081859410430839	0.00821199666280259\\
0.0863945578231292	0.00790807147615624\\
0.0909297052154195	0.00780313069382887\\
0.0954648526077098	0.00885002433216642\\
0.1	0.0111834017579875\\
0.10453514739229	0.0140321973312689\\
0.109070294784581	0.0166299119386963\\
0.113605442176871	0.0183751051772724\\
0.118140589569161	0.0189539188548269\\
0.122675736961451	0.0185365200047953\\
0.127210884353742	0.0178856728879726\\
0.131746031746032	0.0182875558606923\\
0.136281179138322	0.0207525332872107\\
0.140816326530612	0.0249641225232572\\
0.145351473922902	0.0297013768897935\\
0.149886621315193	0.0337782207439414\\
0.154421768707483	0.0363092686417221\\
0.158956916099773	0.036951577703303\\
0.163492063492063	0.0359625337429585\\
0.168027210884354	0.0345866074703388\\
0.172562358276644	0.0349585812623219\\
0.177097505668934	0.0417023425437344\\
0.181632653061225	0.0511230847653164\\
0.186167800453515	0.0594305507756187\\
0.190702947845805	0.0623781475502696\\
0.195238095238095	0.0623902527038722\\
0.199773242630386	0.0615254894345335\\
0.204308390022676	0.0600491371989617\\
0.208843537414966	0.0569335578685286\\
0.213378684807256	0.0575817048501766\\
0.217913832199547	0.0621809306185614\\
0.222448979591837	0.0693231161364491\\
0.226984126984127	0.0728851738713047\\
0.231519274376417	0.0739764213884374\\
0.236054421768708	0.0730384208285301\\
0.240589569160998	0.0706594255106227\\
0.245124716553288	0.0654823244141816\\
0.249659863945578	0.0618648960646255\\
0.254195011337868	0.062635050149912\\
0.258730158730159	0.0671695900325606\\
0.263265306122449	0.0731180684615076\\
0.267800453514739	0.0781603846239197\\
0.272335600907029	0.0816945359553225\\
0.27687074829932	0.0811714143862393\\
0.28140589569161	0.0764950084494338\\
0.2859410430839	0.0701505858342022\\
0.290476190476191	0.0648425606396117\\
0.295011337868481	0.0649941211816527\\
0.299546485260771	0.0697722119666847\\
0.304081632653061	0.0765700008815974\\
0.308616780045352	0.0837059340787943\\
0.313151927437642	0.0874435224755171\\
0.317687074829932	0.086739535014926\\
0.322222222222222	0.0821723863246493\\
0.326757369614513	0.0752187922851598\\
0.331292517006803	0.0700976346722377\\
0.335827664399093	0.0711168005015608\\
0.340362811791383	0.0760743475284771\\
0.349433106575964	0.0916154838289017\\
0.353968253968254	0.0960115251749589\\
0.358503401360544	0.0964985605882963\\
0.363038548752834	0.0935989153619589\\
0.367573696145125	0.0885996862822129\\
0.372108843537415	0.0846574654364893\\
0.376643990929705	0.0840689035869777\\
0.381179138321995	0.087750804119026\\
0.385714285714286	0.0933325605372812\\
0.390249433106576	0.10055318479988\\
0.394784580498866	0.104708764206579\\
0.399319727891156	0.106408963865091\\
0.403854875283447	0.104443372861026\\
0.408390022675737	0.10056568916898\\
0.412925170068027	0.0983714223107737\\
0.417460317460318	0.0981829436214458\\
0.421995464852608	0.101910659454076\\
0.426530612244898	0.107855268401953\\
0.431065759637188	0.115093833384782\\
0.435600907029479	0.120948156909193\\
0.440136054421769	0.124500733907302\\
0.444671201814059	0.12537904896078\\
0.449206349206349	0.125011964560096\\
0.45827664399093	0.126918614700144\\
0.46281179138322	0.130544865152707\\
0.46734693877551	0.135831976393073\\
0.4718820861678	0.142362942822352\\
0.476417233560091	0.147940824747482\\
0.480952380952381	0.15252762352371\\
0.485487528344671	0.155867076556095\\
0.494557823129252	0.159317491586289\\
0.499092970521542	0.161961523096253\\
0.503628117913832	0.166005452539243\\
0.508163265306122	0.171685604438606\\
0.512698412698413	0.177764058373094\\
0.517233560090703	0.182645376286293\\
0.521768707482993	0.186572671030173\\
0.526303854875283	0.189985484384056\\
0.530839002267574	0.192133984031765\\
0.535374149659864	0.194701042513719\\
0.539909297052154	0.198496530325989\\
0.544444444444444	0.203596674998746\\
0.548979591836735	0.209374222117725\\
0.553514739229025	0.214137825607026\\
0.558049886621315	0.216845167599798\\
0.562585034013605	0.217449618754084\\
0.567120181405896	0.217326992967376\\
0.571655328798186	0.218680729824566\\
0.576190476190476	0.222717192612655\\
0.580725623582766	0.230398418376618\\
0.585260770975057	0.239489122882732\\
0.589795918367347	0.246799897383644\\
0.594331065759637	0.248490448732135\\
0.598866213151927	0.244627790988258\\
0.603401360544218	0.236743171170615\\
0.607936507936508	0.229417326515939\\
0.612471655328798	0.229200286109243\\
0.617006802721088	0.239056165609711\\
0.621541950113379	0.256604015107503\\
0.626077097505669	0.275412082553697\\
0.630612244897959	0.287276491469274\\
0.635147392290249	0.286685619683588\\
0.63968253968254	0.273021265301868\\
0.64421768707483	0.250781423186125\\
0.64875283446712	0.229685190484741\\
0.65328798185941	0.223732267563574\\
0.657823129251701	0.239590063100549\\
0.666893424036281	0.302317892737421\\
0.671428571428571	0.322659681849797\\
0.675963718820862	0.324834449988327\\
0.680498866213152	0.307484559404208\\
0.685034013605442	0.274623787327964\\
0.689569160997732	0.237403705433033\\
0.694104308390023	0.215667022771542\\
0.698639455782313	0.226513116510924\\
0.703174603174603	0.265512325275603\\
0.707709750566893	0.31118635176757\\
0.712244897959184	0.345481883778963\\
0.716780045351474	0.357196385611508\\
0.721315192743764	0.342658719284171\\
0.725850340136054	0.304598129069977\\
0.730385487528345	0.253895191108361\\
0.734920634920635	0.212988894218738\\
0.739455782312925	0.210976227027425\\
0.743990929705215	0.250581916701281\\
0.748526077097506	0.305234944058114\\
0.753061224489796	0.350627388924324\\
0.757596371882086	0.373176368749594\\
0.762131519274376	0.367491728798435\\
0.766666666666667	0.334646536239909\\
0.775736961451247	0.229829019241706\\
0.780272108843537	0.206034971122824\\
0.784807256235828	0.231710954347266\\
0.793877551020408	0.341321342183752\\
0.798412698412698	0.376523574119607\\
0.802947845804989	0.383540785749685\\
0.807482993197279	0.360780398224092\\
0.812018140589569	0.313300474216298\\
0.816553287981859	0.254980652917161\\
0.82108843537415	0.212528380792396\\
0.82562358276644	0.216740427209266\\
0.83015873015873	0.264236708828202\\
0.83469387755102	0.322873770425544\\
0.839229024943311	0.368451747579855\\
0.843764172335601	0.388738295760445\\
0.848299319727891	0.379408489617932\\
0.852834467120181	0.342531487958732\\
0.861904761904762	0.232194768999477\\
0.866439909297052	0.209543084907159\\
0.870975056689342	0.239357205495589\\
0.875510204081633	0.298426876802213\\
0.880045351473923	0.354908796378345\\
0.884580498866213	0.389980342064438\\
0.889115646258503	0.395122160744296\\
0.893650793650794	0.369534940136417\\
0.898185941043084	0.318659266498675\\
0.902721088435374	0.25730522484075\\
0.907256235827664	0.214151810249361\\
0.911791383219955	0.222294056624861\\
0.916326530612245	0.275067890533516\\
0.920861678004535	0.336997931713025\\
0.925396825396825	0.383658464516202\\
0.929931972789116	0.402458624651833\\
0.934467120181406	0.389664353002115\\
0.939002267573696	0.348089246330901\\
0.943537414965986	0.288268350745965\\
0.948072562358277	0.23228410697534\\
0.952607709750567	0.214834998055865\\
0.957142857142857	0.25258484801252\\
0.961678004535147	0.316384699667953\\
0.966213151927438	0.373457026352588\\
0.970748299319728	0.406158427385375\\
0.975283446712018	0.407570688464889\\
0.979818594104308	0.377536704092622\\
0.984353741496599	0.322965064678881\\
0.988888888888889	0.26054633216346\\
0.993424036281179	0.222089581973489\\
0.997959183673469	0.239684986916559\\
};
\addlegendentry{ABC$_W^{1/2}$}

\end{axis}
\end{tikzpicture}%

==> images/Linearizations/test_linearizations.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}[scale=0.55][font=\LARGE]

\begin{axis}[%
width=5.358in,
height=4.226in,
at={(0.899in,0.57in)},
% y tick label style={
%         /pgf/number format/.cd,
%             fixed,
%             fixed zerofill,
%             precision=2,
%         /tikz/.cd
%             },
scale only axis,
xmin=2,
xmax=2052,
xlabel style={font=\color{white!15!black}},
xlabel={time step},
ymin=0.0002672729265214,
ymax=0.0430342045560792,  ytick={0.01, 0.02, 0.03, 0.04},
ylabel style={font=\color{white!15!black}},
ylabel={relative error},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.352,0.794)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
2	0.0002672729265214\\
3	0.00048592897837807\\
4	0.000603257132297585\\
5	0.000684160624587093\\
10	0.000957995980115811\\
12	0.00103574733475398\\
15	0.00112302048000856\\
19	0.00120756301521396\\
24	0.00128073366749959\\
31	0.00134908511017784\\
40	0.00140497955908359\\
52	0.00144958555665653\\
68	0.00148048239316267\\
90	0.00149397781024163\\
121	0.00148297022678889\\
220	0.00142650286625212\\
248	0.00144952921027652\\
273	0.00149742517896811\\
296	0.00156842615842834\\
318	0.00166339063116538\\
339	0.00178069785852131\\
360	0.00192539649560786\\
381	0.00209826415766656\\
402	0.00229951529172467\\
423	0.00252879957588448\\
444	0.00278520790834591\\
466	0.00308133963335422\\
489	0.00341867524184636\\
513	0.0037978227937856\\
539	0.00423619284447341\\
566	0.00471875537414235\\
593	0.00522818276022008\\
619	0.00574551324507411\\
644	0.00626982619451155\\
670	0.00684343976718083\\
749	0.00866674845929083\\
769	0.00909802026671969\\
786	0.00943730213884919\\
802	0.00972923997142061\\
818	0.00999321572226108\\
835	0.0102445471779902\\
854	0.0104955274118765\\
931	0.0114061050016971\\
951	0.011674062518523\\
969	0.0119422846723864\\
986	0.0122230203824074\\
1002	0.0125135446610329\\
1018	0.0128304315239802\\
1034	0.0131736774947058\\
1051	0.0135664220856597\\
1068	0.0139864292536913\\
1086	0.0144583138530834\\
1105	0.0149832230003994\\
1126	0.0155906000222785\\
1150	0.0163131951439937\\
1177	0.0171546738888537\\
1207	0.0181180564600254\\
1239	0.0191739602350935\\
1329	0.0222161703431993\\
1349	0.0228627279343527\\
1366	0.023385094848436\\
1381	0.0238189364476966\\
1395	0.0241971270024806\\
1409	0.0245472605033683\\
1423	0.0248685681367533\\
1437	0.0251618329630219\\
1452	0.0254475920646655\\
1469	0.0257416419381116\\
1490	0.0260740155399617\\
1551	0.0270186184548038\\
1569	0.0273368891507744\\
1585	0.027647407310269\\
1600	0.0279654369892341\\
1615	0.0283113424061412\\
1630	0.0286858632612166\\
1645	0.0290888041586186\\
1660	0.0295191504364993\\
1676	0.0300064708408172\\
1693	0.0305532443330776\\
1711	0.0311605760070961\\
1731	0.031863877334672\\
1754	0.0327016761775667\\
1781	0.033713843532496\\
1815	0.0350176362812817\\
1910	0.0387159523911578\\
1932	0.0395435505201931\\
1950	0.0401936123548694\\
1965	0.0407095539335387\\
1979	0.0411650639985055\\
1992	0.0415622408891068\\
2005	0.0419322834668492\\
2018	0.0422738712140927\\
2031	0.042586745848439\\
2052	0.0430342045560792\\
};
\addlegendentry{Linearization \eqref{lin_1}}

\addplot [color=mycolor2][line width=0.7mm]
  table[row sep=crcr]{%
2	0.000267272927885642\\
3	0.000478785993891506\\
4	0.000571800386296673\\
5	0.000617336605500896\\
11	0.000729860490537249\\
17	0.000770821367495955\\
26	0.000794123022387794\\
41	0.000802312833002361\\
65	0.000784887229201559\\
95	0.00073364936042708\\
219	0.000415660739236046\\
254	0.000359780458438763\\
292	0.000328088621245115\\
341	0.000317058230848488\\
399	0.000331854839259904\\
467	0.000378652136078017\\
803	0.000642722357497405\\
1000	0.000633283599654533\\
1081	0.000662290769923857\\
1424	0.000817682451724977\\
1627	0.000790298245647136\\
2052	0.000863758900322864\\
};
\addlegendentry{Linearization \eqref{lin_1/2}}

\end{axis}
\end{tikzpicture}%

==> images/Transducer/Wave.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.602in,
height=3.82in,
at={(0.772in,0.516in)},
scale only axis,
xmin=-0.005,
xmax=0.01,
xlabel style={font=\color{white!15!black}},
xlabel={$y$\,[m]},
ymin=-40000000,
ymax=40000000,
ylabel style={font=\color{white!15!black}},
ylabel={pressure\,[Pa]},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]
\addplot [color=blue, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
-0.00499960035085678	25077000\\
-0.00485710054636002	26203000\\
-0.00476709753274918	26777000\\
-0.00471460074186325	27036000\\
-0.00466209650039673	27256000\\
-0.00457960367202759	27480000\\
-0.00457210093736649	27496000\\
-0.00454960018396378	27503000\\
-0.00443709641695023	27549000\\
-0.00442209839820862	27529000\\
-0.00436209887266159	27429000\\
-0.00432460010051727	27334000\\
-0.00426460057497025	27079000\\
-0.00421959906816483	26865000\\
-0.00411459803581238	26232000\\
-0.00409209728240967	26046000\\
-0.00397209823131561	24943000\\
-0.00386709719896317	23721000\\
-0.00377710163593292	22512000\\
-0.00364209711551666	20404000\\
-0.00348459929227829	17411000\\
-0.00332710146903992	13996000\\
-0.00313960015773773	9274000\\
-0.00305719673633575	7022200\\
-0.00287719815969467	1838900\\
-0.00266720354557037	-4709800\\
-0.00214970111846924	-20779000\\
-0.00202970206737518	-24196000\\
-0.00194720178842545	-26344000\\
-0.00185719877481461	-28570000\\
-0.00175219774246216	-30979000\\
-0.0016172006726265	-33671000\\
-0.00148969888687134	-35744000\\
-0.00135470181703568	-37534000\\
-0.00124970078468323	-38493000\\
-0.00115969777107239	-39108000\\
-0.00113719701766968	-39216000\\
-0.00105469673871994	-39537000\\
-0.00102470070123672	-39608000\\
-0.000934712588787079	-39695000\\
-0.000919707119464874	-39671000\\
-0.000829711556434631	-39498000\\
-0.000814713537693024	-39471000\\
-0.000799708068370819	-39424000\\
-0.000784710049629211	-39364000\\
-0.000612221658229828	-38400000\\
-0.00046221911907196	-36962000\\
-0.000349722802639008	-35696000\\
-0.000244729220867157	-34277000\\
-0.000117227435112	-32335000\\
2.52649188041687e-05	-29953000\\
0.000145256519317627	-27758000\\
0.000302761793136597	-24657000\\
0.000557750463485718	-19374000\\
0.000872738659381866	-12358000\\
0.00112020224332809	-6587100\\
0.00147269666194916	1443100\\
0.00187770277261734	10380000\\
0.00218520313501358	16813000\\
0.00242520123720169	21529000\\
0.00258269906044006	24417000\\
0.00273270159959793	27022000\\
0.0028752014040947	29240000\\
0.00313019752502441	32959000\\
0.00325769931077957	34462000\\
0.00336270034313202	35542000\\
0.00342269986867905	36111000\\
0.0035426989197731	37037000\\
0.00360269844532013	37330000\\
0.00366269797086716	37603000\\
0.0037676990032196	37846000\\
0.00379019975662231	37853000\\
0.00382769852876663	37803000\\
0.00389520078897476	37713000\\
0.00391770154237747	37630000\\
0.00394769757986069	37498000\\
0.00403019785881042	36991000\\
0.00409770011901855	36360000\\
0.00417269766330719	35422000\\
0.00422520190477371	34572000\\
0.00433769822120667	32347000\\
0.00448010116815567	28137000\\
0.00461509823799133	22936000\\
0.00475010275840759	16556000\\
0.00486259907484055	10489000\\
0.00508759915828705	-1798400\\
0.0052001029253006	-7451700\\
0.00531259924173355	-12444000\\
0.00544010102748871	-17216000\\
0.00556010007858276	-20868000\\
0.00569509714841843	-24119000\\
0.00582259893417358	-26463000\\
0.00587510317564011	-27193000\\
0.00595010071992874	-28159000\\
0.00604759901762009	-29144000\\
0.0060850977897644	-29399000\\
0.00617510080337524	-29986000\\
0.00632510334253311	-30435000\\
0.00636260211467743	-30451000\\
0.00638510286808014	-30461000\\
0.00642260164022446	-30477000\\
0.00643759965896606	-30484000\\
0.00644510239362717	-30485000\\
0.00646010041236877	-30488000\\
0.00647509843111038	-30459000\\
0.00650510191917419	-30384000\\
0.00661010295152664	-30099000\\
0.00665509700775146	-29908000\\
0.0067375972867012	-29472000\\
0.00681260228157043	-29008000\\
0.00691760331392288	-28257000\\
0.00707510113716125	-26908000\\
0.00733009725809097	-24113000\\
0.00747259706258774	-22395000\\
0.0076150968670845	-20526000\\
0.00799009948968887	-15219000\\
0.00864250212907791	-5677000\\
0.0088450014591217	-2496900\\
0.00934000313282013	5684400\\
0.00940749794244766	6711600\\
0.00965499877929688	10054000\\
0.00970000028610229	10631000\\
0.00975249707698822	11355000\\
0.00980500131845474	12055000\\
0.00997749716043472	14968000\\
0.00999999791383743	15389000\\
};
\end{axis}
\end{tikzpicture}%

==> images/Transducer3D/Cost_V.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.60000,0.00000}%
%
\begin{tikzpicture}[scale = 0.52, font=\huge]

\begin{axis}[%
width=4.602in,
height=3.82in,
at={(0.772in,0.516in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\huge\color{white!15!black}},
xlabel={relative simulation time $t/T$}, xtick={0, 0.2, 0.4, 0.6, 0.8, 1},
y tick label style={
        /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=2,
        /tikz/.cd
            },
ymin=0.02,
ymax=0.22,
ylabel style={font=\huge\color{white!15!black}},
ylabel={relative $L^{2}(\Omega)$ error},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
0.00428571428571434	0.213078877670931\\
0.0083673469387755	0.142326950718768\\
0.0124489795918368	0.104326690962522\\
0.0165306122448979	0.0755083333294011\\
0.0206122448979592	0.056669679193567\\
0.0246938775510204	0.0478964587146894\\
0.0287755102040816	0.0491863024185218\\
0.0328571428571428	0.0599019686400597\\
0.0369387755102041	0.077888574773333\\
0.0410204081632654	0.0941536284645343\\
0.0451020408163265	0.0905627310531868\\
0.0491836734693878	0.0731105806634808\\
0.053265306122449	0.0565558300993804\\
0.0573469387755102	0.0449271165558626\\
0.0614285714285714	0.0378566152396218\\
0.0655102040816327	0.0345170260401974\\
0.0695918367346939	0.0343031175139542\\
0.0736734693877551	0.0367193906578154\\
0.0777551020408164	0.0413637533058365\\
0.0818367346938775	0.0475587751605654\\
0.0859183673469388	0.0534545718241158\\
0.09	0.0559067591154188\\
0.0940816326530612	0.0532058384188121\\
0.0981632653061224	0.0473074296386327\\
0.102244897959184	0.0411010798380629\\
0.106326530612245	0.036099972045413\\
0.110408163265306	0.0326983541522093\\
0.114489795918367	0.0309624746331748\\
0.118571428571429	0.0308807459426427\\
0.12265306122449	0.0324085469103773\\
0.126734693877551	0.0353567235158936\\
0.130816326530612	0.0391779668806845\\
0.134897959183674	0.0427814413164015\\
0.138979591836735	0.0446932098790445\\
0.143061224489796	0.0439365307028142\\
0.147142857142857	0.0409901605065368\\
0.151224489795918	0.0372126957950613\\
0.15530612244898	0.0337318429293265\\
0.159387755102041	0.0311639232855673\\
0.163469387755102	0.0297778567412308\\
0.167551020408163	0.0296796654138258\\
0.171632653061225	0.030845795323926\\
0.175714285714286	0.0330773221078525\\
0.183877551020408	0.0387372535446748\\
0.187959183673469	0.040494376991816\\
0.192040816326531	0.040514702293823\\
0.196122448979592	0.0388441267113554\\
0.200204081632653	0.0362099038501378\\
0.204285714285714	0.0345350781843849\\
0.208367346938776	0.0337978799277859\\
0.216530612244898	0.0340382002031316\\
0.220612244897959	0.0351149341641812\\
0.22469387755102	0.0366052334625319\\
0.228775510204082	0.0382893562195389\\
0.232857142857143	0.0398284331970592\\
0.236938775510204	0.0408487625688178\\
0.241020408163265	0.0408469029164039\\
0.245102040816327	0.0399414484829582\\
0.253265306122449	0.0371296906181311\\
0.25734693877551	0.0362452451108223\\
0.261428571428571	0.0360092764548966\\
0.265510204081633	0.0364570817520469\\
0.269591836734694	0.0376078602399174\\
0.273673469387755	0.0392506929309602\\
0.277755102040816	0.0412110778828103\\
0.281836734693878	0.0429834443501528\\
0.285918367346939	0.0441784912271956\\
0.29	0.0446876841376649\\
0.294081632653061	0.0447092191518804\\
0.298163265306122	0.0445124801263449\\
0.302244897959184	0.0441924541795233\\
0.306326530612245	0.044023958798927\\
0.310408163265306	0.0442736687399674\\
0.314489795918367	0.0450691461808774\\
0.318571428571429	0.0464517512011456\\
0.32265306122449	0.0482411181619127\\
0.330816326530612	0.052041380706895\\
0.334897959183673	0.0536050338576515\\
0.338979591836735	0.0546506618550718\\
0.343061224489796	0.0551576444208974\\
0.347142857142857	0.0549693025394408\\
0.35530612244898	0.0535140667080519\\
0.359387755102041	0.0532483864468474\\
0.363469387755102	0.0540159888121363\\
0.367551020408163	0.0559742159400102\\
0.371632653061225	0.0589717898189706\\
0.375714285714286	0.0625594768954476\\
0.379795918367347	0.0659547341125886\\
0.383877551020408	0.0683320001581168\\
0.387959183673469	0.0690389655916502\\
0.392040816326531	0.0678320803601432\\
0.396122448979592	0.0651032851363985\\
0.400204081632653	0.0617433371447309\\
0.404285714285714	0.0590852318728928\\
0.408367346938776	0.0586960611264162\\
0.412448979591837	0.0617671762999101\\
0.416530612244898	0.0678474086702607\\
0.420612244897959	0.0752748702701843\\
0.42469387755102	0.0821409610902569\\
0.428775510204082	0.0869181371576424\\
0.432857142857143	0.088463398087157\\
0.436938775510204	0.0861372702366658\\
0.441020408163265	0.0800400275651244\\
0.445102040816327	0.0713338836839584\\
0.449183673469388	0.0623533059668401\\
0.453265306122449	0.0566660618344251\\
0.45734693877551	0.0576265232323609\\
0.461428571428571	0.0652252786440262\\
0.465510204081633	0.0766550001138985\\
0.469591836734694	0.0887679849538041\\
0.473673469387755	0.099069986098661\\
0.477755102040816	0.105645801381019\\
0.481836734693878	0.107166817024397\\
0.485918367346939	0.102926217369459\\
0.49	0.0930253976118951\\
0.494081632653061	0.0785974530885971\\
0.498163265306122	0.062391488693414\\
0.502244897959184	0.0497809087067312\\
0.506326530612245	0.0483347418851625\\
0.510408163265306	0.0590193170892835\\
0.518571428571429	0.0911340779600831\\
0.52265306122449	0.104522522095338\\
0.526734693877551	0.11333135938753\\
0.530816326530612	0.11620564333438\\
0.534897959183673	0.112477951740813\\
0.538979591836735	0.102237278557596\\
0.543061224489796	0.0863914831783007\\
0.547142857142857	0.0671173959072149\\
0.551224489795918	0.049075102431654\\
0.55530612244898	0.0412977277038173\\
0.559387755102041	0.0501786503887202\\
0.563469387755102	0.0676649564137098\\
0.567551020408163	0.086123099969695\\
0.571632653061224	0.102087940596001\\
0.575714285714286	0.113632938271925\\
0.579795918367347	0.119276769499084\\
0.583877551020408	0.118084289472344\\
0.587959183673469	0.109788990330272\\
0.592040816326531	0.0950329648937799\\
0.596122448979592	0.0754911204030148\\
0.600204081632653	0.0547462058975626\\
0.604285714285714	0.0400685144227984\\
0.608367346938775	0.0424521506215247\\
0.612448979591837	0.0585203885456285\\
0.616530612244898	0.07777266364559\\
0.620612244897959	0.0954819683603046\\
0.62469387755102	0.109355066939365\\
0.628775510204082	0.117780590266565\\
0.632857142857143	0.119614005117319\\
0.636938775510204	0.114415094875561\\
0.641020408163265	0.102514544500776\\
0.645102040816326	0.0850551526166977\\
0.649183673469388	0.0646343787203285\\
0.653265306122449	0.0462313833146344\\
0.65734693877551	0.0398249939189229\\
0.661428571428571	0.0505909455563641\\
0.665510204081633	0.0689116962048162\\
0.669591836734694	0.0875780339218213\\
0.673673469387755	0.103444320562404\\
0.677755102040816	0.114584861389542\\
0.681836734693878	0.119615753049206\\
0.685918367346939	0.117760639336927\\
0.69	0.109059862324138\\
0.694081632653061	0.0942572270106877\\
0.702244897959184	0.0562156555117619\\
0.706326530612245	0.0444040758320967\\
0.710408163265306	0.0481984582419859\\
0.714489795918367	0.0633144557255126\\
0.718571428571429	0.0813290877693225\\
0.72265306122449	0.0978839056685823\\
0.726734693877551	0.110600535667421\\
0.730816326530612	0.117881834351579\\
0.734897959183674	0.118825464697691\\
0.738979591836735	0.113167549217325\\
0.743061224489796	0.101277829836363\\
0.747142857142857	0.0845196092313375\\
0.751224489795918	0.065996136200637\\
0.75530612244898	0.0513747180493679\\
0.759387755102041	0.0486402651846747\\
0.763469387755102	0.0590736214535716\\
0.767551020408163	0.0754464674551879\\
0.771632653061225	0.0921637396652538\\
0.775714285714286	0.106230083702556\\
0.779795918367347	0.115637277276871\\
0.783877551020408	0.119195300620462\\
0.787959183673469	0.116313346941188\\
0.792040816326531	0.107159443955586\\
0.796122448979592	0.0926313948470455\\
0.800204081632653	0.0752528917284013\\
0.804285714285714	0.059579716632855\\
0.808367346938776	0.0523763631687583\\
0.812448979591837	0.0576026444196928\\
0.816530612244898	0.0709733626619348\\
0.820612244897959	0.0866405028841353\\
0.82469387755102	0.100922635153973\\
0.828775510204082	0.11150267441683\\
0.832857142857143	0.116947954280238\\
0.836938775510204	0.116570277029786\\
0.841020408163265	0.110227469534808\\
0.845102040816327	0.0984365809377401\\
0.853265306122449	0.0672636131270619\\
0.85734693877551	0.05713257344337\\
0.861428571428571	0.0576008724016417\\
0.865510204081633	0.0675032931781657\\
0.873673469387755	0.0956888121691167\\
0.877755102040816	0.107166698590366\\
0.881836734693878	0.11425979707705\\
0.885918367346939	0.11602569887209\\
0.89	0.112139082019068\\
0.894081632653061	0.102880423844254\\
0.898163265306122	0.0895529127582987\\
0.902244897959184	0.0751621110804997\\
0.906326530612245	0.0642082719376157\\
0.910408163265306	0.0613301385599586\\
0.914489795918367	0.0672602389003419\\
0.918571428571429	0.0784809958198424\\
0.92265306122449	0.0911711116920099\\
0.926734693877551	0.102503799596207\\
0.930816326530612	0.1105246691852\\
0.934897959183673	0.114073589833295\\
0.938979591836735	0.112611707877546\\
0.943061224489796	0.106102669513692\\
0.947142857142857	0.0953009341926361\\
0.951224489795918	0.0823844802641457\\
0.95530612244898	0.0711436606782724\\
0.959387755102041	0.065679104607384\\
0.963469387755102	0.0680740797189703\\
0.967551020408163	0.0764139560016998\\
0.975714285714286	0.0984988474647249\\
0.979795918367347	0.107351612559781\\
0.983877551020408	0.112601696203901\\
0.987959183673469	0.113379499574298\\
0.992040816326531	0.109459445970411\\
0.996122448979592	0.101150302822244\\
};
\addlegendentry{ABC$_W^{1/2}$ adaptive}

\addplot [color=mycolor1, dashed]
  table[row sep=crcr]{%
0.00428571428571434	0.213078877670931\\
0.0083673469387755	0.142326950718768\\
0.0124489795918368	0.104326690962522\\
0.0165306122448979	0.0755083333294011\\
0.0206122448979592	0.056669679193567\\
0.0246938775510204	0.0478964587146894\\
0.0287755102040816	0.0491863024185218\\
0.0328571428571428	0.0599019686400597\\
0.0369387755102041	0.077888574773333\\
0.0410204081632654	0.0941536284645343\\
0.0451020408163265	0.0905627310531868\\
0.0491836734693878	0.0731105806634808\\
0.053265306122449	0.0565558300993804\\
0.0573469387755102	0.0449271165558626\\
0.0614285714285714	0.0378566152396218\\
0.0655102040816327	0.0345170260401974\\
0.0695918367346939	0.0343031175139542\\
0.0736734693877551	0.0367193906578154\\
0.0777551020408164	0.0413637533058365\\
0.0818367346938775	0.0475587751605654\\
0.0859183673469388	0.0534545718241158\\
0.09	0.0559067591154188\\
0.0940816326530612	0.0532058384188121\\
0.0981632653061224	0.0473074296386327\\
0.102244897959184	0.0411010798380629\\
0.106326530612245	0.036099972045413\\
0.110408163265306	0.0326983541522093\\
0.114489795918367	0.0309624746331748\\
0.118571428571429	0.0308807459426427\\
0.12265306122449	0.0324085469103773\\
0.126734693877551	0.0353567235158936\\
0.130816326530612	0.0391779668806845\\
0.134897959183674	0.0427814413164015\\
0.138979591836735	0.0446932098790445\\
0.143061224489796	0.0439365307028142\\
0.147142857142857	0.0409901605065368\\
0.151224489795918	0.0372126957950613\\
0.15530612244898	0.0337318429293265\\
0.159387755102041	0.0311639232855673\\
0.163469387755102	0.0297778567412308\\
0.167551020408163	0.0296796654138258\\
0.171632653061225	0.030845795323926\\
0.175714285714286	0.0330773221078525\\
0.183877551020408	0.0387372535446748\\
0.187959183673469	0.040494376991816\\
0.192040816326531	0.040514702293823\\
0.196122448979592	0.0388441267113554\\
0.200204081632653	0.0362099038501378\\
0.204285714285714	0.0345350781843849\\
0.208367346938776	0.0337978799277859\\
0.216530612244898	0.0340382002031316\\
0.220612244897959	0.0351149341641812\\
0.22469387755102	0.0366052334625319\\
0.228775510204082	0.0382879577675201\\
0.232857142857143	0.0398104935485296\\
0.236938775510204	0.0407792002772649\\
0.241020408163265	0.0406922933365995\\
0.245102040816327	0.0396807709013521\\
0.253265306122449	0.0366767978137456\\
0.25734693877551	0.035723686649082\\
0.261428571428571	0.0354264142996715\\
0.265510204081633	0.0358183264487618\\
0.269591836734694	0.036895281184627\\
0.273673469387755	0.0384511719407252\\
0.277755102040816	0.0403320457748864\\
0.281836734693878	0.0420197358926085\\
0.285918367346939	0.0431434940254921\\
0.29	0.0435932885444056\\
0.294081632653061	0.0435798321827854\\
0.302244897959184	0.0431520193236319\\
0.306326530612245	0.0431100098589646\\
0.310408163265306	0.0435018868815491\\
0.314489795918367	0.0444558802517852\\
0.318571428571429	0.0460344773992606\\
0.32265306122449	0.0480717540385607\\
0.326734693877551	0.0503572970655142\\
0.330816326530612	0.0527350552740004\\
0.334897959183673	0.0549372013522642\\
0.338979591836735	0.056720630772237\\
0.343061224489796	0.058016588508742\\
0.347142857142857	0.0586584937751042\\
0.351224489795918	0.0586469425930685\\
0.35530612244898	0.0583304549372007\\
0.359387755102041	0.0581530724810744\\
0.363469387755102	0.0586228672777664\\
0.367551020408163	0.0601470019842802\\
0.371632653061225	0.0630106685393299\\
0.375714285714286	0.0672043669666079\\
0.383877551020408	0.0771883147261989\\
0.387959183673469	0.0811278061030843\\
0.392040816326531	0.0831476335763075\\
0.396122448979592	0.0827926279826349\\
0.400204081632653	0.0801713941447775\\
0.404285714285714	0.0760370487769142\\
0.408367346938776	0.071744804080618\\
0.412448979591837	0.0693336576900871\\
0.416530612244898	0.0706817033015141\\
0.420612244897959	0.0765373780802071\\
0.42469387755102	0.0859359644960476\\
0.428775510204082	0.0968032472269249\\
0.432857142857143	0.106738757258817\\
0.436938775510204	0.113539907603024\\
0.441020408163265	0.115543614011635\\
0.445102040816327	0.111898141396566\\
0.449183673469388	0.102807694261308\\
0.453265306122449	0.0897112727152378\\
0.45734693877551	0.0755929045471032\\
0.461428571428571	0.0655903458754062\\
0.465510204081633	0.0660454354924113\\
0.469591836734694	0.0781506713648873\\
0.473673469387755	0.0966424037586969\\
0.477755102040816	0.115837255577226\\
0.481836734693878	0.131695677487867\\
0.485918367346939	0.141278364865946\\
0.49	0.142680340498832\\
0.494081632653061	0.135142782218785\\
0.498163265306122	0.119304552086155\\
0.502244897959184	0.0972067888455252\\
0.506326530612245	0.0727104208534509\\
0.510408163265306	0.0536243022112954\\
0.514489795918367	0.0533271858302189\\
0.518571428571429	0.0723754714330134\\
0.52265306122449	0.0977349298464492\\
0.526734693877551	0.121668599913204\\
0.530816326530612	0.140337497010243\\
0.534897959183673	0.151324607805105\\
0.538979591836735	0.15311430176\\
0.543061224489796	0.145206588538169\\
0.547142857142857	0.128233800176663\\
0.551224489795918	0.104080318874178\\
0.55530612244898	0.0759647033364427\\
0.559387755102041	0.0503703437411133\\
0.563469387755102	0.0433253940659283\\
0.567551020408163	0.062637745378175\\
0.571632653061224	0.0906599649096618\\
0.575714285714286	0.117499328497396\\
0.579795918367347	0.139107848777252\\
0.583877551020408	0.153036707757804\\
0.587959183673469	0.157561602355757\\
0.592040816326531	0.151983931329925\\
0.596122448979592	0.136728147294978\\
0.600204081632653	0.113520572125633\\
0.608367346938775	0.0568131032872969\\
0.612448979591837	0.0409313906673788\\
0.616530612244898	0.0536695291990107\\
0.620612244897959	0.0807755336646626\\
0.62469387755102	0.108547631340977\\
0.628775510204082	0.132059132034463\\
0.632857142857143	0.148672009097932\\
0.636938775510204	0.156585299942615\\
0.641020408163265	0.154815881185687\\
0.645102040816326	0.143377899687357\\
0.649183673469388	0.123428832559286\\
0.653265306122449	0.0971658394855645\\
0.65734693877551	0.0683422384418672\\
0.661428571428571	0.0452737871591943\\
0.665510204081633	0.0462225331158914\\
0.669591836734694	0.0698687385455513\\
0.673673469387755	0.0983346218661005\\
0.677755102040816	0.124168975036488\\
0.681836734693878	0.144066520672779\\
0.685918367346939	0.155812399260739\\
0.69	0.158019352794108\\
0.694081632653061	0.150253853541334\\
0.698163265306122	0.13327354515156\\
0.702244897959184	0.109080210491201\\
0.706326530612245	0.0809931007032478\\
0.710408163265306	0.0553093877764455\\
0.714489795918367	0.0463168668628924\\
0.718571428571429	0.0627523934284857\\
0.726734693877551	0.115464530652567\\
0.730816326530612	0.136927747161508\\
0.734897959183674	0.151279063408408\\
0.738979591836735	0.156886898227907\\
0.743061224489796	0.15295834814394\\
0.747142857142857	0.139732067055846\\
0.751224489795918	0.118717135240128\\
0.759387755102041	0.0663463335552396\\
0.763469387755102	0.0501533336388074\\
0.767551020408163	0.057305903055717\\
0.771632653061225	0.0805448588418596\\
0.775714285714286	0.106795571014649\\
0.779795918367347	0.130018100996593\\
0.783877551020408	0.147119902256854\\
0.787959183673469	0.156022944302646\\
0.792040816326531	0.155598098640623\\
0.796122448979592	0.145688088026743\\
0.800204081632653	0.127487580439629\\
0.804285714285714	0.103432607202236\\
0.808367346938776	0.0776568783303361\\
0.812448979591837	0.0578431965877001\\
0.816530612244898	0.0564023713713531\\
0.820612244897959	0.0740390098311455\\
0.82469387755102	0.0983573710602058\\
0.828775510204082	0.12158332827413\\
0.832857142857143	0.140001016688774\\
0.836938775510204	0.151322496467431\\
0.841020408163265	0.154133474558492\\
0.845102040816327	0.147909722637006\\
0.849183673469388	0.133193530716802\\
0.853265306122449	0.111873703383668\\
0.85734693877551	0.0873135717100074\\
0.861428571428571	0.0655540497013641\\
0.865510204081633	0.0570817834566417\\
0.869591836734694	0.0681559159062436\\
0.873673469387755	0.0898972315680957\\
0.877755102040816	0.113051103139865\\
0.881836734693878	0.132908758824321\\
0.885918367346939	0.14675000117752\\
0.89	0.152775429738739\\
0.894081632653061	0.15003320086343\\
0.898163265306122	0.138696731991434\\
0.902244897959184	0.120346452148165\\
0.906326530612245	0.0979408654319182\\
0.910408163265306	0.0764106044478419\\
0.914489795918367	0.0636683578298537\\
0.918571428571429	0.0672917513515332\\
0.92265306122449	0.0839959045662585\\
0.926734693877551	0.105059471354797\\
0.930816326530612	0.12482995163135\\
0.934897959183673	0.140129736827331\\
0.938979591836735	0.148825761989544\\
0.943061224489796	0.14961036151155\\
0.947142857142857	0.142121942577631\\
0.951224489795918	0.127239225766278\\
0.95530612244898	0.107267511972573\\
0.959387755102041	0.0860659974115083\\
0.963469387755102	0.0700228297473076\\
0.967551020408163	0.0669306497793757\\
0.971632653061224	0.0783674164719823\\
0.975714285714286	0.0973954487406431\\
0.979795918367347	0.117452638265032\\
0.983877551020408	0.134613531816884\\
0.987959183673469	0.146215091982774\\
0.992040816326531	0.150495967606585\\
0.996122448979592	0.146523627067845\\
};
\addlegendentry{ABC$_W^{1/2}$}

\end{axis}
\end{tikzpicture}%

==> images/Transducer3D/Cost_V_abs.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.60000,0.00000}%
%
\begin{tikzpicture}[scale = 0.52, font=\huge]

\begin{axis}[%
width=4.602in,
height=3.82in,
at={(0.772in,0.516in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\huge\color{white!15!black}},
xlabel={relative simulation time $t/T$}, xtick={0, 0.2, 0.4, 0.6, 0.8, 1},
y tick label style={
        /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=2,
        /tikz/.cd
            },
ymin=0,
ymax=0.35,
ylabel style={font=\huge\color{white!15!black}},
ylabel={absolute $L^{2}(\Omega)$ error},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.03,0.97)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
0.000204081632653064	0\\
0.0287755102040816	0.00069328296761062\\
0.0369387755102041	0.00117679985101071\\
0.0491836734693878	0.00205410926741578\\
0.0695918367346939	0.00300882811712677\\
0.0777551020408164	0.0039875863338783\\
0.0940816326530612	0.00639476657858296\\
0.102244897959184	0.00725028239469816\\
0.114489795918367	0.00831640143692847\\
0.118571428571429	0.00890188656161073\\
0.12265306122449	0.00971483945638463\\
0.126734693877551	0.0107501181236155\\
0.138979591836735	0.0143096898673263\\
0.143061224489796	0.0153034494474021\\
0.147142857142857	0.0160820089485846\\
0.15530612244898	0.0171119967190996\\
0.159387755102041	0.0175777390121421\\
0.163469387755102	0.0182239401614801\\
0.167551020408163	0.0192081633002332\\
0.171632653061225	0.0206113474433601\\
0.175714285714286	0.0223895555945358\\
0.187959183673469	0.0283425403010178\\
0.192040816326531	0.0299236890779984\\
0.196122448979592	0.0311196673880941\\
0.200204081632653	0.0319548236928644\\
0.204285714285714	0.0333175451389131\\
0.208367346938776	0.035033068966439\\
0.212448979591837	0.0370751408335512\\
0.216530612244898	0.0384072913695261\\
0.22469387755102	0.042243411912408\\
0.236938775510204	0.0482557649370426\\
0.241020408163265	0.0495826797732223\\
0.245102040816327	0.050333824638107\\
0.253265306122449	0.0509889468744242\\
0.25734693877551	0.0516923040287334\\
0.261428571428571	0.0529106772954976\\
0.265510204081633	0.0546908382703625\\
0.269591836734694	0.0570979391431821\\
0.273673469387755	0.0599131952402338\\
0.277755102040816	0.0630201856257131\\
0.281836734693878	0.0658695195898961\\
0.285918367346939	0.0681047149741159\\
0.29	0.0697309706980096\\
0.302244897959184	0.0738589068052939\\
0.306326530612245	0.0754309081129105\\
0.310408163265306	0.077470953950882\\
0.314489795918367	0.0800924675887715\\
0.318571428571429	0.0833292621321861\\
0.326734693877551	0.0903754732582568\\
0.330816326530612	0.0936978699243455\\
0.334897959183673	0.0965845728521045\\
0.338979591836735	0.0989103977886588\\
0.343061224489796	0.10076150040795\\
0.347142857142857	0.101824644381622\\
0.35530612244898	0.102578201445372\\
0.359387755102041	0.103654412270817\\
0.363469387755102	0.106359912982508\\
0.367551020408163	0.110938080792695\\
0.371632653061225	0.117063349310832\\
0.375714285714286	0.123895896045752\\
0.379795918367347	0.130046759166822\\
0.383877551020408	0.134173728124922\\
0.387959183673469	0.135324379788965\\
0.392040816326531	0.133248723795696\\
0.396122448979592	0.128730576525925\\
0.400204081632653	0.123317985533561\\
0.404285714285714	0.119384520010981\\
0.408367346938776	0.11986831306867\\
0.412448979591837	0.127082602672925\\
0.416530612244898	0.139987256694084\\
0.420612244897959	0.154990787176284\\
0.42469387755102	0.168118567669461\\
0.428775510204082	0.176465643449576\\
0.432857142857143	0.178192619306415\\
0.436938775510204	0.172576967312003\\
0.441020408163265	0.16014374797071\\
0.449183673469388	0.12602566215877\\
0.453265306122449	0.115564417940499\\
0.45734693877551	0.118564604333952\\
0.461428571428571	0.135086304787832\\
0.465510204081633	0.159212830455417\\
0.469591836734694	0.184095593782417\\
0.473673469387755	0.204336896414126\\
0.477755102040816	0.216146774362262\\
0.481836734693878	0.217360587384283\\
0.485918367346939	0.207309628411229\\
0.49	0.186752047361059\\
0.494081632653061	0.158000807780123\\
0.498163265306122	0.126126486745428\\
0.502244897959184	0.101474871267341\\
0.506326530612245	0.0994046555766261\\
0.510408163265306	0.122266252376442\\
0.518571428571429	0.189563118673932\\
0.52265306122449	0.216556013871885\\
0.526734693877551	0.233226869849629\\
0.530816326530612	0.237271688386606\\
0.534897959183673	0.228114631824957\\
0.538979591836735	0.206556758971903\\
0.543061224489796	0.174590597598873\\
0.547142857142857	0.136237085658492\\
0.551224489795918	0.10035495343497\\
0.55530612244898	0.0851758412911966\\
0.559387755102041	0.104274154274171\\
0.563469387755102	0.141278416175453\\
0.567551020408163	0.179953077971828\\
0.571632653061224	0.212593063892355\\
0.575714285714286	0.235032024376675\\
0.579795918367347	0.244610295568343\\
0.583877551020408	0.240200644517725\\
0.587959183673469	0.22208701405598\\
0.592040816326531	0.191946633288056\\
0.596122448979592	0.152919829790312\\
0.600204081632653	0.111612737270058\\
0.604285714285714	0.0823590393940407\\
0.608367346938775	0.0879373869018055\\
0.612448979591837	0.121890090419529\\
0.616530612244898	0.162311186009642\\
0.620612244897959	0.198890720765916\\
0.62469387755102	0.226603378912795\\
0.628775510204082	0.242292809917613\\
0.632857142857143	0.244237406187829\\
0.636938775510204	0.232288780178943\\
0.641020408163265	0.207621835487075\\
0.645102040816326	0.172526065939845\\
0.649183673469388	0.131779049570484\\
0.653265306122449	0.0949633048343975\\
0.65734693877551	0.082453002087295\\
0.661428571428571	0.10542132391438\\
0.669591836734694	0.183044586394215\\
0.673673469387755	0.215281783576538\\
0.677755102040816	0.236774642775717\\
0.681836734693878	0.245103025190131\\
0.685918367346939	0.239494396698385\\
0.69	0.220762673515288\\
0.694081632653061	0.190671036063133\\
0.702244897959184	0.114868020878666\\
0.706326530612245	0.0914554352984479\\
0.710408163265306	0.0999970018168184\\
0.714489795918367	0.132002865271582\\
0.718571428571429	0.169802523531373\\
0.72265306122449	0.203892105341361\\
0.726734693877551	0.22911991717707\\
0.730816326530612	0.24241626750638\\
0.734897959183674	0.242558756828522\\
0.738979591836735	0.229740235864353\\
0.743061224489796	0.205172474491655\\
0.747142857142857	0.171565247802775\\
0.751224489795918	0.134723429431512\\
0.75530612244898	0.105702180594616\\
0.759387755102041	0.100887021263596\\
0.763469387755102	0.123299018355331\\
0.771632653061225	0.192744855241679\\
0.775714285714286	0.22108435732335\\
0.779795918367347	0.238844800787102\\
0.783877551020408	0.244086739561825\\
0.787959183673469	0.236426330897099\\
0.792040816326531	0.216871644617253\\
0.796122448979592	0.187450497154105\\
0.800204081632653	0.152908865396537\\
0.804285714285714	0.121927211110257\\
0.808367346938776	0.108077033383398\\
0.812448979591837	0.119746330275863\\
0.816530612244898	0.148267349143807\\
0.820612244897959	0.181227789191838\\
0.82469387755102	0.210556473848564\\
0.828775510204082	0.231258941147727\\
0.832857142857143	0.240635867331349\\
0.836938775510204	0.23795529344358\\
0.841020408163265	0.223673842772055\\
0.845102040816327	0.199308091569962\\
0.853265306122449	0.13740515295445\\
0.85734693877551	0.117763164568549\\
0.861428571428571	0.119822482040172\\
0.865510204081633	0.141421435408529\\
0.873673469387755	0.200845146518197\\
0.877755102040816	0.223618717999875\\
0.881836734693878	0.236270104464318\\
0.885918367346939	0.237518889225848\\
0.89	0.227589845659168\\
0.894081632653061	0.207788051008253\\
0.898163265306122	0.180927194599505\\
0.902244897959184	0.15268935645792\\
0.906326530612245	0.131645871222024\\
0.910408163265306	0.127069750272172\\
0.914489795918367	0.140629087132066\\
0.918571428571429	0.165002692713206\\
0.92265306122449	0.191831834226168\\
0.926734693877551	0.214780871288258\\
0.930816326530612	0.22968559038389\\
0.934897959183673	0.234604636844002\\
0.938979591836735	0.22929201157629\\
0.943061224489796	0.214557945546633\\
0.947142857142857	0.192393610907829\\
0.951224489795918	0.167019578770757\\
0.95530612244898	0.145550238692682\\
0.959387755102041	0.135950591244931\\
0.963469387755102	0.142518236420302\\
0.967551020408163	0.161289479465784\\
0.971632653061224	0.185178973793227\\
0.975714285714286	0.207871374869657\\
0.979795918367347	0.224583940272284\\
0.983877551020408	0.232635793171373\\
0.987959183673469	0.231150242571727\\
0.992040816326531	0.220800210771862\\
0.996122448979592	0.203032630951183\\
};
\addlegendentry{ABC$_W^{1/2}$ adaptive}

\addplot [color=mycolor1, dashed]
  table[row sep=crcr]{%
0.000204081632653064	0\\
0.0287755102040816	0.00069328296761062\\
0.0369387755102041	0.00117679985101071\\
0.0491836734693878	0.00205410926741578\\
0.0695918367346939	0.00300882811712677\\
0.0777551020408164	0.0039875863338783\\
0.0940816326530612	0.00639476657858296\\
0.102244897959184	0.00725028239469816\\
0.114489795918367	0.00831640143692847\\
0.118571428571429	0.00890188656161073\\
0.12265306122449	0.00971483945638463\\
0.126734693877551	0.0107501181236155\\
0.138979591836735	0.0143096898673263\\
0.143061224489796	0.0153034494474021\\
0.147142857142857	0.0160820089485846\\
0.15530612244898	0.0171119967190996\\
0.159387755102041	0.0175777390121421\\
0.163469387755102	0.0182239401614801\\
0.167551020408163	0.0192081633002332\\
0.171632653061225	0.0206113474433601\\
0.175714285714286	0.0223895555945358\\
0.187959183673469	0.0283425403010178\\
0.192040816326531	0.0299236890779984\\
0.196122448979592	0.0311196673880941\\
0.200204081632653	0.0319548236928644\\
0.204285714285714	0.0333175451389131\\
0.208367346938776	0.035033068966439\\
0.212448979591837	0.0370751408335512\\
0.216530612244898	0.0384072913695261\\
0.22469387755102	0.042243411912408\\
0.232857142857143	0.0463213735091809\\
0.236938775510204	0.048173589091838\\
0.241020408163265	0.0493950044113717\\
0.245102040816327	0.0500053212868765\\
0.253265306122449	0.0503670045216015\\
0.25734693877551	0.0509484669132551\\
0.261428571428571	0.0520542415534049\\
0.265510204081633	0.0537326139334862\\
0.269591836734694	0.0560160696809443\\
0.273673469387755	0.0586927873032104\\
0.277755102040816	0.0616759653466451\\
0.281836734693878	0.0643926948709171\\
0.285918367346939	0.0665091831335528\\
0.29	0.0680232682623563\\
0.298163265306122	0.0706675428431325\\
0.302244897959184	0.0721200266619533\\
0.306326530612245	0.073864942661574\\
0.310408163265306	0.0761204745685471\\
0.314489795918367	0.0790026315099608\\
0.318571428571429	0.0825807194590022\\
0.326734693877551	0.0907349481034484\\
0.334897959183673	0.0989848479601532\\
0.338979591836735	0.102656765024795\\
0.343061224489796	0.105984194359045\\
0.347142857142857	0.10865846923064\\
0.351224489795918	0.110484211219789\\
0.359387755102041	0.113201975721555\\
0.363469387755102	0.115431064015762\\
0.367551020408163	0.119208332863863\\
0.371632653061225	0.125080821256603\\
0.375714285714286	0.133094867104321\\
0.383877551020408	0.151563600224334\\
0.387959183673469	0.159019909270876\\
0.392040816326531	0.163334457705725\\
0.396122448979592	0.16370821702732\\
0.400204081632653	0.160123752303447\\
0.404285714285714	0.153636471983587\\
0.408367346938776	0.146516281868794\\
0.412448979591837	0.142650226218983\\
0.416530612244898	0.145835160657818\\
0.420612244897959	0.157590287893978\\
0.42469387755102	0.175885831753226\\
0.428775510204082	0.196534899027178\\
0.432857142857143	0.215004839840328\\
0.436938775510204	0.227478452349124\\
0.441020408163265	0.23117917328113\\
0.445102040816327	0.224597275759065\\
0.449183673469388	0.207790229297353\\
0.453265306122449	0.182956617742924\\
0.45734693877551	0.155529820564437\\
0.461428571428571	0.13584238562507\\
0.465510204081633	0.137176710035656\\
0.469591836734694	0.162076386626335\\
0.477755102040816	0.236998052139277\\
0.481836734693878	0.267111132060747\\
0.485918367346939	0.284556899801079\\
0.49	0.286436246340998\\
0.494081632653061	0.271671255455975\\
0.498163265306122	0.24117815302189\\
0.502244897959184	0.198149182903073\\
0.506326530612245	0.149535387174325\\
0.510408163265306	0.111089771807396\\
0.514489795918367	0.110922911495124\\
0.518571428571429	0.150544345073062\\
0.52265306122449	0.202493074213135\\
0.526734693877551	0.250384243779447\\
0.530816326530612	0.286544731427163\\
0.534897959183673	0.306898878058\\
0.538979591836735	0.30934698546357\\
0.543061224489796	0.293451439140708\\
0.547142857142857	0.260293162194988\\
0.551224489795918	0.212836551256545\\
0.55530612244898	0.156675872375409\\
0.559387755102041	0.104672504210766\\
0.563469387755102	0.0904595728457683\\
0.567551020408163	0.130880740265789\\
0.571632653061224	0.18879487234238\\
0.575714285714286	0.243029050023834\\
0.579795918367347	0.285279456747371\\
0.583877551020408	0.311298954353318\\
0.587959183673469	0.318723996748674\\
0.592040816326531	0.306975626460451\\
0.596122448979592	0.276965620595792\\
0.600204081632653	0.231437806212778\\
0.608367346938775	0.117685341536834\\
0.612448979591837	0.0852545759424311\\
0.616530612244898	0.112008056925597\\
0.62469387755102	0.22493022704183\\
0.628775510204082	0.271665968929978\\
0.632857142857143	0.303570353983194\\
0.636938775510204	0.31790393004685\\
0.641020408163265	0.313547288054115\\
0.645102040816326	0.290828059379924\\
0.649183673469388	0.251651436376249\\
0.653265306122449	0.199587132657503\\
0.65734693877551	0.141494628734148\\
0.661428571428571	0.0943414385410655\\
0.665510204081633	0.096649443837362\\
0.669591836734694	0.146030845592771\\
0.673673469387755	0.204647801518381\\
0.677755102040816	0.256578961230692\\
0.681836734693878	0.295204763130061\\
0.685918367346939	0.316881742228936\\
0.69	0.319868135229268\\
0.694081632653061	0.303945478090034\\
0.698163265306122	0.270538421500803\\
0.702244897959184	0.222888584720513\\
0.706326530612245	0.166814850713149\\
0.710408163265306	0.11474999723436\\
0.714489795918367	0.0965649797703391\\
0.718571428571429	0.131017266442397\\
0.72265306122449	0.186046032126672\\
0.726734693877551	0.23919616248114\\
0.730816326530612	0.281582939114703\\
0.734897959183674	0.308806379574292\\
0.738979591836735	0.31849442046049\\
0.743061224489796	0.309868831446668\\
0.747142857142857	0.283640292808425\\
0.751224489795918	0.242347211709649\\
0.759387755102041	0.137611995714572\\
0.763469387755102	0.104680509722474\\
0.767551020408163	0.119966485018667\\
0.771632653061225	0.168445933447605\\
0.775714285714286	0.222261240505694\\
0.779795918367347	0.268547895302788\\
0.783877551020408	0.301270411497793\\
0.787959183673469	0.317142728907019\\
0.792040816326531	0.314902861622682\\
0.796122448979592	0.294816941655013\\
0.800204081632653	0.259046274893064\\
0.804285714285714	0.211670179832256\\
0.808367346938776	0.160242608000787\\
0.812448979591837	0.120246398278799\\
0.816530612244898	0.117827728249097\\
0.820612244897959	0.154868977198748\\
0.82469387755102	0.205204523205877\\
0.828775510204082	0.252166433719619\\
0.832857142857143	0.288070589054044\\
0.836938775510204	0.308895114337953\\
0.841020408163265	0.312768012363921\\
0.845102040816327	0.299478143822058\\
0.849183673469388	0.270329283106679\\
0.853265306122449	0.228534011337984\\
0.85734693877551	0.179973032801424\\
0.861428571428571	0.13636683986714\\
0.865510204081633	0.119588058182741\\
0.869591836734694	0.143256872096456\\
0.873673469387755	0.188688962027911\\
0.877755102040816	0.235897373765706\\
0.881836734693878	0.274833030820713\\
0.885918367346939	0.300415318437361\\
0.89	0.310062610186522\\
0.894081632653061	0.303022725111791\\
0.898163265306122	0.280214343078465\\
0.902244897959184	0.244479859151596\\
0.910408163265306	0.158314927265991\\
0.914489795918367	0.133119108513374\\
0.918571428571429	0.141477819622457\\
0.92265306122449	0.176734583371803\\
0.926734693877551	0.220135886509147\\
0.930816326530612	0.259413951196683\\
0.934897959183673	0.288191912496701\\
0.938979591836735	0.303028512613127\\
0.943061224489796	0.302538022328129\\
0.947142857142857	0.286915904375872\\
0.951224489795918	0.257954432952218\\
0.95530612244898	0.219454717718038\\
0.959387755102041	0.178149859138972\\
0.963469387755102	0.146598092048306\\
0.967551020408163	0.141272749482858\\
0.971632653061224	0.165904851092182\\
0.979795918367347	0.245715696932329\\
0.983877551020408	0.27811238019997\\
0.987959183673469	0.298093165928271\\
0.992040816326531	0.303578563487631\\
0.996122448979592	0.294107646443472\\
};
\addlegendentry{ABC$_W^{1/2}$}

\end{axis}
\end{tikzpicture}%
